Variable Selection for Kernel Two-Sample Tests

We consider the variable selection problem for two-sample tests, aiming to select the most informative variables to determine whether two collections of samples follow the same distribution. To address this, we propose a novel framework based on the kernel maximum mean discrepancy (MMD). Our approach seeks a subset of variables with a pre-specified size that maximizes the variance-regularized kernel MMD statistic. We focus on three commonly used types of kernels: linear, quadratic, and Gaussian. From a computational perspective, we derive mixed-integer programming formulations and propose exact and approximation algorithms with performance guarantees to solve these formulations. From a statistical viewpoint, we derive the rate of testing power of our framework under appropriate conditions. These results show that the sample size requirements for the three kernels depend crucially on the number of selected variables, rather than the data dimension. Experimental results on synthetic and real datasets demonstrate the superior performance of our method, compared to other variable selection frameworks, particularly in high-dimensional settings.

==> cover.tex <==
Dear Editor,

I, together with my coauthors Jie Wang and Yao Xie, are hereby submitting our paper "Sinkhorn Distributionally Robust Optimization" to Operations Research.

In this work, we study distributionally robust optimization in which the ambiguity set is constructed using Sinkhorn distance --- a variant of Wasserstein distance with entropic regularization. 
This is motivated by two potential issues in the recently popular Wasserstein DRO framework. First, Wasserstein DRO is shown to be tractable under certain conditions so that the inner maximization subproblem can be evaluated efficiently (Esfahani & Kuhn [2018], Blanchet et al. [2021]). 
Second, for data-driven Wasserstein DRO, the worst-case distribution is often a discrete distribution (Gao & Kleywegt [2016]), despite that the underlying true distribution is often continuous. 

We develop a strong dual reformulation of the Sinkhorn DRO problem and establish the worst-case distribution. Compared with Wasserstein DRO, Sinkhorn DRO is tractable for a broader class of loss functions and yield a more reasonable worst-case distribution. On the algorithmic aspect, we propose a computationally efficient first-order algorithm for solving the Sinkhorn DRO dual problem. 

 
There are no relevant or material financial interests that relate to the research described in their paper.

Thank you very much for your consideration！

Sincerely,
Rui Gao

==> premeable.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[english]{babel}
\usepackage{microtype}
\usepackage[smallerops,vvarbb]{newtxmath}
\usepackage[varqu,varl]{inconsolata}%
\usepackage[scaled=0.95]{helvet}
\DeclareMathAlphabet{\mathsfit}{T1}{\sfdefault}{\mddefault}{\sldefault}
\SetMathAlphabet{\mathsfit}{bold}{T1}{\sfdefault}{\bfdefault}{\sldefault}
\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}
\usepackage{mathtools,accents}
\usepackage{xifthen,enumitem,comment}
\setlist[enumerate,1]{label=\normalfont{(\Roman*)},leftmargin=2em}
\usepackage{xcolor}
\usepackage{etoolbox}
\makeatletter
\patchcmd{\env@cases}{1.2}{0.96}{}{}
\makeatother
\usepackage{algorithm,algpseudocode}
\usepackage[hypertexnames=false]{hyperref}
\hypersetup{%
  colorlinks=true,%
  linkcolor={blue!66!black},%
  linkbordercolor=red,%
  citecolor={blue!66!black},
}
\usepackage{booktabs,tikz,pgfplots,subfigure}
\usetikzlibrary{matrix,decorations.pathreplacing}

\newcommand{\TBA}{{\color{red}{TBA}}}
\ifx\argmax\undefined\DeclareMathOperator*{\argmax}{arg\,max}\fi
\ifx\argmin\undefined\DeclareMathOperator*{\argmin}{arg\,min}\fi
\DeclareMathOperator*{\esssupOp}{-ess\,sup}
\DeclareMathOperator*{\tsum}{\textstyle{\sum\limits}}
\providecommand\esssup[2]{\underset{#2}{#1\!\esssupOp}}
\providecommand{\Norm}[1]{\lVert\hspace{1pt}#1\hspace{1pt}\rVert}
\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\dist}[2]{\norm{#1-#2}}
\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\diam}{\mathrm{diam}}
\providecommand{\inner}[2]{\left\langle#1,#2\right\rangle}
\providecommand{\Cov}{\mathbb{C}\mathrm{ov}}
\newcommand*{\QED}{%
\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
    \quad\hbox{$\square$}%
}
\newcommand*{\QEG}{%
\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
    \quad\hbox{$\clubsuit$}%
}
\newcommand*{\QDEF}{%
\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
    \quad\hbox{$\diamondsuit$}%
}

\providecommand{\1}{1}
\providecommand{\allOne}{\boldsymbol{1}}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\hP}{\hat{\mathbb{P}}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hy}{\hat{y}}
\newcommand{\hz}{\hat{z}}
\providecommand{\hxi}{\hat{\xi}}
\providecommand{\hXi}{\hat{\Xi}}
\providecommand{\E}{\mathbb{E}}
\providecommand{\R}{\mathbb{R}}
\providecommand{\CVaR}{\mathbb{C}\textrm{V@R}}
\providecommand{\Var}{\mathbb{V}\textrm{ar}}
\providecommand{\Q}{\mathbb{Q}}
\providecommand{\N}{\mathbb{N}}
\providecommand{\frakM}{\mathfrak{M}}
\providecommand{\cA}{\mathcal{A}}
\providecommand{\cB}{\mathcal{B}}
\providecommand{\cC}{\mathcal{C}}
\providecommand{\cD}{\mathcal{D}}
\providecommand{\cE}{\mathcal{E}}
\providecommand{\cF}{\mathcal{F}}
\providecommand{\cG}{\mathcal{G}}
\providecommand{\cH}{\mathcal{H}}
\providecommand{\cI}{\mathcal{I}}
\providecommand{\cJ}{\mathcal{J}}
\providecommand{\cK}{\mathcal{K}}
\providecommand{\cL}{\mathcal{L}}
\providecommand{\cM}{\mathcal{M}}
\providecommand{\cN}{\mathcal{N}}
\providecommand{\cO}{\mathcal{O}}
\providecommand{\cP}{\mathcal{P}}
\providecommand{\cQ}{\mathcal{Q}}
\providecommand{\cR}{\mathcal{R}}
\providecommand{\cS}{\mathcal{S}}
\providecommand{\cT}{\mathcal{T}}
\providecommand{\cU}{\mathcal{U}}
\providecommand{\cV}{\mathcal{V}}
\providecommand{\cW}{\mathcal{W}}
\providecommand{\cX}{\mathcal{X}}
\providecommand{\cY}{\mathcal{Y}}
\providecommand{\cZ}{\mathcal{Z}}
\providecommand{\bxi}{\boldsymbol{\xi}}
\providecommand{\Rad}{\mathfrak{R}}
\providecommand{\VCdim}{\mathrm{VCdim}}
\providecommand{\Dirac}{\boldsymbol{\updelta}}
\providecommand{\bbsigma}{\boldsymbol{\sigma}}
\providecommand{\tr}{\mathrm{tr}}
\providecommand{\conv}{\mathrm{conv}}

\definecolor{longhorn}{rgb}{0.8, 0.33, 0.0}
\newcommand{\rgao}[1]{{\textcolor{longhorn}{#1}}}
